Diffusion-Reward Adversarial Imitation Learning

Imitation learning aims to learn a policy from observing expert demonstrations without access to reward signals from environments. Generative adversarial imitation learning (GAIL) formulates imitation learning as adversarial learning, employing a generator policy learning to imitate expert behaviors and discriminator learning to distinguish the expert demonstrations from agent trajectories. Despite its encouraging results, GAIL training is often brittle and unstable. Inspired by the recent dominance of diffusion models in generative modeling, we propose Diffusion-Reward Adversarial Imitation Learning (DRAIL), which integrates a diffusion model into GAIL, aiming to yield more robust and smoother rewards for policy learning. Specifically, we propose a diffusion discriminative classifier to construct an enhanced discriminator, and design diffusion rewards based on the classifier's output for policy learning. Extensive experiments are conducted in navigation, manipulation, and locomotion, verifying DRAIL's effectiveness compared to prior imitation learning methods. Moreover, additional experimental results demonstrate the generalizability and data efficiency of DRAIL. Visualized learned reward functions of GAIL and DRAIL suggest that DRAIL can produce more robust and smoother rewards. Project page: https://nturobotlearninglab.github.io/DRAIL/

==> figure/diffusion_model.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figure/diffusion_model_fig.pdf}
    \caption[]{\textbf{Denoising diffusion probabilistic model.} 
    Latent variables $\mathbf{x}_1, ..., \mathbf{x}_T$ are produced from the data point $\mathbf{x}_0$ via the forward diffusion process, i.e., gradually adding noises to the latent variables. The diffusion model $\phi$ learns to reverse the process by denoising the noisy data to reconstruct the original data point $\mathbf{x}_0$.
    }
    \label{fig:dm}
\end{figure}

==> figure/walker_traj.tex <==
\begin{figure*}[t]
    % \vspace{-10pt}
    \centering
    
    % \begin{subfigure}[b]{0.7\textwidth}
    % \label{fig:result_legend}
    % \includegraphics[trim={0 2.75cm 0 2.75cm},clip,width=\textwidth]{figure/training_curve/legend.pdf}
    % \end{subfigure}
    \begin{subfigure}[b]{0.7\textwidth}
    \label{fig:traj_legend}
    \centering
    \includegraphics[trim={0 2.75cm 0cm 2.75cm},clip,width=\textwidth]
    {figure/walker_sample/legend.pdf}
    \end{subfigure}

    \begin{subfigure}[b]{0.23\textwidth}
    \label{fig:walker_1traj}
    \centering
    \includegraphics[width=\textwidth, height=0.75\textwidth]{figure/sa}
    \caption{\walker{} 1 trajectory}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \label{fig:walker_2traj}
    \centering
    \includegraphics[width=\textwidth, height=0.75\textwidth]{figure/walker_sample/walker_2traj.png}
    \caption{\walker{} 2 trajectories}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \label{fig:walker_3traj}
    \centering
    \includegraphics[width=\textwidth, height=0.75\textwidth]{figure/walker_sample/walker_3traj.png}
    \caption{\walker{} 3 trajectories}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.23\textwidth}
    \label{fig:walker_5traj}
    \centering
    \includegraphics[width=\textwidth, height=0.75\textwidth]{figure/walker_sample/walker_5traj.png}
    \caption{\walker{} 5 trajectories}
    \end{subfigure}
    \vspace{-0.3cm}

    \caption{\textbf{Sample efficiency and data efficiency.}  
    We report the full training curves of BC, GAIL, and \method{} using varying amounts of expert data in \walker{}. Our \method{} demonstrates superior sample efficiency in terms of environment interaction and data efficiency in terms of expert demonstration.
    }
    \label{fig:walker_sample}
\end{figure*}


==> table/ablation_result.tex <==
\begin{table}
\centering
\caption[Ablation Study]{\textbf{Effect of the dimension of the conditional vector.}
We report the result of performance under different conditional vector dimensionality.
}
\scalebox{0.9}{\begin{tabular}{@{}ccc@{}}\toprule
\textbf{Environment}  & $\textbf{Dim}(\textbf{c}) = 1$ & $\textbf{Dim}(\textbf{c}) = 10$ \\
\cmidrule{1-3}
\fetchpush{} 1.00 &  98.8\% $\pm$ 1.4\% & 98.4\% $\pm$ 1.5\%\\
\fetchpush{} 1.25 &  96.4\% $\pm$ 2.2\% & 94.9\% $\pm$ 2.5\%\\
\fetchpush{} 1.50 &  96.1\% $\pm$ 1.8\% & 97.0\% $\pm$ 1.9\%\\
\fetchpush{} 1.75 &  97.3\% $\pm$ 2.1\% & 98.3\% $\pm$ 1.5\%\\
\fetchpush{} 2.00 &  99.1\% $\pm$ 0.8\% & 98.5\% $\pm$ 1.3\%\\
\walker &  5908 $\pm$ 531 & 5441 $\pm$ 1078\\
\bottomrule
\end{tabular}}
\label{table:abla_result}
\end{table}




==> table/hp.tex <==
\begin{table*}
\centering
\small
\caption[Hyperparameters]{\textbf{Hyperparameters.}
This table presents the overview of the hyperparameters used for all the methods across various tasks. }
%\ra{1.3}
\scalebox{0.75}{\begin{tabular}{@{}cccccccc@{}}\toprule
\textbf{Method} & \textbf{Hyperparameter} & 
\maze{} &
\fetchpick{} &
\fetchpush{} &
\handrotate{} &
\walker{} &
\antreach{} \\
% & Success Rate & Episode Length & Success Rate & Episode Length & Success Rate & Episode Length & Return\\
\cmidrule{1-8}
\multirow{3}{*}{BC} 
& Learning Rate & 0.00005 & 0.0008 & 0.0002 & 0.0001 & 0.0001 & 0.001 \\
& Batch Size & 128 & 128 & 128 & 128 & 128 & 128 \\
& \# Epochs & 2000 & 1000 & 1000 & 5000 & 1000 & 1000 \\
\cmidrule{1-8}
\multirow{3}{*}{Diffusion Policy} 
& Learning Rate & 0.0002 & 0.00001 & 0.0001 & 0.0001 & 0.0001 & 0.00001 \\
& Batch Size & 128 & 128 & 128 & 128 & 128 & 128 \\
& \# Epochs & 20000 & 20000 & 10000 & 2000 & 5000 & 10000 \\
\cmidrule{1-8}
\multirow{3}{*}{GAIL} 
& Discriminator Learning Rate & 0.001 & 0.00001 & 0.000008 & 0.0001 & 0.0000005 & 0.0001 \\
& Policy Learning Rate & 0.0001 & 0.00005 & 0.0002 & 0.0001 & 0.0001 & 0.0001 \\
& Environment Step & 25000000 & 25000000 & 5000000 & 5000000 & 25000000 & 10000000 \\
\cmidrule{1-8}
\multirow{3}{*}{WAIL} 
& Discriminator Learning Rate & 0.00001 & 0.0001 & 0.00008 & 0.0001 & 0.0000008 & 0.00001 \\
& Policy Learning Rate & 0.00001 & 0.0005 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
& Environment Step & 25000000 & 25000000 & 5000000 & 5000000 & 25000000 & 10000000 \\
\cmidrule{1-8}
\multirow{3}{*}{\method{} (Ours)}
& Discriminator Learning Rate & 0.001 & 0.0001 & 0.001 & 0.0001 & 0.0002 & 0.001 \\
& Policy Learning Rate & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
& Environment Step & 25000000 & 25000000 & 5000000 & 5000000 & 25000000 & 10000000 \\
\cmidrule{1-8}
\multirow{3}{*}{\methodnn{}} 
& Discriminator Learning Rate & 0.001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
& Policy Learning Rate & 0.0001 & 0.0001 & 0.00005 & 0.0001 & 0.0001 & 0.0001 \\
& Environment Step & 25000000 & 25000000 & 5000000 & 5000000 & 25000000 & 10000000 \\
\bottomrule
\end{tabular}}
\label{table:hyperparameter}
\end{table*}



